Quasi-periodic solutions of nonlinear wave equations on the d-dimensional torus

The main result of this research Monograph is the existence of small amplitude time quasi-periodic solutions for autonomous nonlinear wave equations $$ u_{tt} - \Delta u + V(x) u + g(x, u) = 0 \, , \quad x \in T^d \, , \quad g (x,u) = a(x) u^3 + O(u^4 ) , $$ in any space dimension and with a multiplicative potential. The proof is based on a Nash-Moser implicit function scheme. A key step is the construction of an approximate right inverse of the linearized operators obtained at any step of the iteration. In order to avoid the difficulty posed by the violation of the second order Melnikov non-resonance conditions we develop a multiscale inductive approach \'a la Bourgain. A feature of the Monograph is to present the proofs, techniques and ideas developed in a self-contained and expanded manner.

==> Abstract.tex <==

\chapter*{Abstract}
% \pagestyle{plain}

\thispagestyle{empty}

The main result of this research Monograph 
is to prove the existence of  small amplitude
time quasi-periodic solutions  for {\it autonomous} nonlinear wave equations (NLW)
$$
u_{tt} - \Delta u + V(x) u + g(x, u) = 0 \, , \quad x \in \T^d \, ,  
$$
in {\it any} space dimension $ d \geq 1 $,
where $ V(x)  $ is a smooth {\it multiplicative} potential,  
 and $ g (x,u)  $ is a smooth 
nonlinearity of the form 
$ g (x,u) = a(x) u^3 + O(u^4 ) $. 
This is a 
difficult small divisor problem, due to complex resonance phenomena among 
the linear normal mode frequencies of oscillations 
$ \mu_j $ where $ (\mu_j^2)_j $ denote the eigenvalues of $ - \Delta + V(x) $, and the fact that the corresponding 
eigenfunctions $ \Psi_j (x) $ are not in general ``localized with respect to exponentials". 

 %The solutions have Sobolev regularity both in time and space. 
The proof is based on  a Nash-Moser iterative scheme in scales of Sobolev spaces for the search of an invariant  torus embedding supporting quasi-periodic solutions, with a 
frequency 
$ \omega $ to be determined.
One key step is to establish the existence of an  % key tame estimates for the 
approximate inverse of the  operators obtained 
linearizing the nonlinear wave equation at each approximate solution,
satisfying tame estimates 
in Sobolev spaces. These are  linear operators of the form
$$
h \mapsto h_{tt} - \Delta h + V(x) h + (\pa_u g)(x, u(\omega t,x)) h 
$$
with coefficients depending on $ x \in \T^d $ and quasi-periodically  on time.
% acting on functions $ h $ % (\om t , x) $ which are quasi-periodic in time. 
The construction of an approximate inverse requires several tools. 
%Much of this material is inspired to works
%in Anderson localization and we think 
We first use 
a symplectic reduction to approximately decouple the action-angle and normal components of the linearized operator. This step is a rather general procedure for autonomous PDEs, which reduces the problem to the search of an approximate inverse for a  quasi-periodic 
Hamiltonian  linear operator acting in the subspace normal to the torus. 
In order to avoid the difficulty posed by the violation of 
the second order Melnikov non-resonance conditions required by 
a KAM reducibility scheme, we develop a 
%Since the second order Melnikov non-resonance conditions required by 
%a KAM reducibility schemes are strongly violated, we develop a 
% Then we prove a general 
multiscale inductive approach {\' a la} Bourgain,  which is particularly delicate since the eigenfunctions $ \Psi_j (x) $ of $ - \Delta + V(x) $ are not localized near the exponentials. 
% in presence of a  multiplicative potential. 
The presence of a multiplicative potential makes also difficult to control the variations of the 
tangential and normal frequencies with respect to parameters. 
%to obtain the existence of an approximate inverse 
%for a class of Hamiltonian linearized operator acting in the normal subspace. 
In this Monograph, after a careful bifurcation analysis of the quasi-periodic solutions, 
we are able to use 
just the frequency length as an internal parameter to verify the %  Melnikov % required 
non-resonance conditions along the iteration. 

The 
techniques developed in this Monograph  
have deep connections with those used in Anderson localization theory.  
% are an extension of  
All the proofs % This Monograph 
are presented % all proofs 
in a % detailed and 
self-contained manner.    
%Many of the techniques developed in this Monograph 
%have deep connections with the the Anderson localization results.  
% Much of this material has certainly deep connections with the 
%field of Anderson localization.  


